Resource Allocation to Agents with Restrictions: Maximizing Likelihood with Minimum Compromise

Many scenarios where agents with restrictions compete for resources can be cast as maximum matching problems on bipartite graphs. Our focus is on resource allocation problems where agents may have restrictions that make them incompatible with some resources. We assume that a Principle chooses a maximum matching randomly so that each agent is matched to a resource with some probability. Agents would like to improve their chances of being matched by modifying their restrictions within certain limits. The Principle's goal is to advise an unsatisfied agent to relax its restrictions so that the total cost of relaxation is within a budget (chosen by the agent) and the increase in the probability of being assigned a resource is maximized. We establish hardness results for some variants of this budget-constrained maximization problem and present algorithmic results for other variants. We experimentally evaluate our methods on synthetic datasets as well as on two novel real-world datasets: a vacation activities dataset and a classrooms dataset.

==> scratch.tex <==
\section{Additional material for Section~\ref{sec:definitions}}
\textbf{Estimating number of maximum matchings.}~ Algorithms
for finding a maximum matching and enumerating all maximum
matchings in bipartite graphs form an important component
of our advice generation methods. We have
two requirements: the \prin{} needs to 
(i)~sample uniformly from the space
of maximum matchings of the compatibility graph for assigning
resources to agents, and 
(ii)~compute the probability that an
agent will be matched in such a maximum matching. 
%Both problems are known
%to be hard~\cite{}. 
%\textcolor{red}{(We need to think about the next sentence
%that informally talks about the hardness of (i) and (ii) above. I thought %that (i) is not difficult.)}
These problems are closely related to the computationally difficult 
problem of counting the number of maximum matchings
in bipartite graphs \cite{Jerrum-1987,miklos2020counting}.
Therefore, we use use the following heuristic methods 
in our experiments.

For~(i), we use the following method based on
the matching algorithm by Hopcroft and Karp~(\citeyear{Hopcroft-Karp-1973}), which we refer
to as the HK-algorithm.
We randomly permute the node labels
of~$V_{\sagset}$, apply the HK-algorithm to 
find a maximum matching, and apply the
inverse of the permutation to obtain 
the original labels. We refer to this
as the \emph{random HK-algorithm} (\rhk{} algorithm). 
For~(ii) we use a
combination of \rhk{} algorithm and the iterative algorithm developed by
 Uno~(\citeyear{uno1997algorithms}) 
to enumerate all maximum matchings in a bipartite graph, 
which we refer to as the \hkuno{} algorithm.
Let~$\trueprob$ be the probability that~$x_i$ is matched. The notation
\hkuno{}$(\nhk,\nuno)$ corresponds to~$\nhk$ iterations of first
running~\rhk{} algorithm followed by running the Uno algorithm
for ~$\nuno$ steps. This which will 
provide~$\nhk(\nuno+1)$ matchings, and we keep track of
how many of these matchings contain $x_i$.
From these values, we can
compute an empirical estimate $\empprob$ of~$\trueprob$.
Using appropriate values of $\nhk$ and $\nuno$,
we will refer to \hkuno{}$(\nhk,\nuno)$ as the
``matching oracle".
 During the running of the
algorithms,following the relaxations of constraints, additional edges
became compatible and were added to the graph.


\section{Additional Material for Section~\ref{sec:preliminaries}}
\label{sec:sup_preliminaries}

%\subsection{Statement and Proof of Lemma~\ref{lem:oracle_calls}}

\begin{lemma} \label{lem:oracle_calls}
For an agent~$x_i\in\agset$, suppose the set \rset{} of resources can be
partitioned into~$\eta$ subsets~$\rset=
\rset_0\uplus\rset_1\uplus\cdots\uplus\rset_\eta$ such that for every pair of
resources~$y_a,y_b\in\rset_{\ell}$, $\kappa'_i(\attvec(y_a))=
\kappa'_i(\attvec(y_b))$ for every
extension~$\kappa'_i$ of~$\kappa_i$. Then, to evaluate any extension
of~$\kappa_i$, it suffices to know the number of new maximum matchings
obtained by adding exactly~$\rset_l$ to the original compatibility graph,
for all~$\ell=1,2,\ldots,\eta$. Further, let~$\distattset=\{A_i\mid \forall
y_i\in \rset\}$ be the collection of distinct attribute value sets among
the resources in~$\rset$.  Then,~$\eta\le|\distattset|\le m$, where~$m$ is
the number of resources.
\end{lemma}
%%

\medskip
The following example illustrates the concepts presented in
the statement of Lemma~\ref{lem:oracle_calls}.

\textbf{Example 2:}~
Consider a scenario where the compatibility functions belong to the class
$\compatand$ of conjunction of variables. Let $y_1$, $y_2$, $y_3$ and
$y_4$ be four resources with the following 
attribute values: $A_1=\{a1,a2,a4\}$, $A_2=\{a1,a2\}$, $A_3=\{a3,a4\}$,
$A_4=\{a3,a4\}$. For agent~$x_i$, let~$\kappa_i= (b_{a3}\And b_{a5})$. None
of the above resources is compatible with~$x_i$.  Any extension
of~$\kappa_i$ corresponds to removing one or both of the variables 
in $\kappa_i$.
For each resource $y_j$, let $B_j$ denote the set of Boolean
variables corresponding to the attribute value set $A_j$, $1 \leq j \leq 4$.
Thus, for any two resources~$y_j$ and~$y_{j'}$,
if~$\Gamma_i\setminus B_j=\Gamma_i\setminus B_{j'}$, then, for any
extension~$\kappa'_i$,~$\kappa'_i(\attvec(y_j)) =\kappa'_i(\attvec(y_{j'}))$. 
For example,~$y_1$ and~$y_2$ belong to the same class as both~$a3$ and~$a5$
need to be removed for them to be compatible with~$x_i$, while~$y_3$
and~$y_4$ will become compatible with $x_i$ if~$b_{a5}$ is removed from $\kappa_i$.




\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Additional Material for Section~\ref{sec:customer_side}}
\label{sec:sup_customer_side}


\subsection{Statement and Proof of Theorem~\ref{thm:or_greedy}}

\underline{Statement of Theorem~\ref{thm:or_greedy}:}~
Consider the \problem{} for a customer~$x_i$
under~$\frameworkor(\forbidden,\attvec,\compatibilityset,\kappa_i,\chi)$ framework
where~$\chi(b) = 1$ for each $b \in \boolattribs - \Gamma_i$.
Algorithm~\ref{alg:or_greedy} provides an extension~$\kappa^g_i$ with cost
at most~$\beta$ and benefit at least~$(1-1/e)$ of the optimal
solution~$\kappa^*_i$.
The algorithm uses at most $m = |\rset|$ calls to the matching
oracle. The other parts of the algorithm run in polynomial time.

\smallskip

\noindent
\textbf{Proof.~}
There are two parts to Algorithm~\ref{alg:or_greedy}. The first part
handles Matching scenario~1. For each incompatible resource~$y_j$, it
checks whether making it compatible increases the maximum matching size in
the resulting graph~$G_j$. If this is indeed the case, then by Part~1 of
Definition~\ref{def:matching_scenarios},~$x_i$ is matched in all maximum
matchings of~$G'$. Therefore, this is the best benefit one can obtain after
extending~$\kappa_i$, which can be realized by adding any variable
from~$B_j$ to~$\Gamma_i$. 
%% If not, then, we will make
%% all~$y_j$ such that~$M(G_j)>M(G)$ forbidden. This will ensure that the
%%maximum matching size never increases. 
Otherwise, we have Matching scenario~$2$. For this case, by
Lemma~\ref{lem:or_submodular},~$\extor(\cdot)$ is submodular. It follows from
the analysis in 
Nemhauser~et.~al.~(\citeyear{nemhauser1978analysis}) that
Algorithm~\ref{alg:or_greedy} provides stated approximation ratio
for \problem{}. We will complete the proof by bounding the 
number of calls to the matching oracle and the time for the
other steps of the algorithm.

To check for Matching scenario~1, we need to compute at most~$m$ maximum
matchings, one for each~$G_j$. Since a maximum matching in
a bipartite graph with $q$ nodes can be computed in $O(q^{2.5})$ time
\cite{Hopcroft-Karp-1973}, the time used for computing the matchings is
$O\big(m((n+m)^{2.5})\big)$
computations. Matching scenario~2 requires at most~$m$ calls to the oracle
that computes number of maximum matchings (by
Lemma~\ref{lem:oracle_calls}). In each iteration~$\ell$, at
most~$|\boolattribs|-\ell$ variables will be evaluated to identify~$b^*$.
To compute~$\benefit(\kappa_i^b)$, we need to find the set of resources
that become compatible for each node; this can be done in $O(m)$ time. 
Once we have
this set, by Lemma~\ref{lem:oracle_calls}, the benefit can be computed
in time~$O(\beta\,m|\boolattribs|)$ since each variable has
unit cost. Hence, the algorithm uses at most $m$ calls to the matching
oracle and the other parts of the algorithm run in time
$O\big(m(n+m)^{2.5} + \beta\,m|\boolattribs|\big)$ time.
\QED
%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi


\subsection{The~$\frameworkand$ framework with uniform costs}
\label{sec:supp_conjunction}
We recall that~$x_i$ and~$y_j$ are compatible only if~$\Gamma_i\subseteq
B_j$. Therefore,~$\kappa'_i$ is an extension of~$\kappa_i$
iff~$\Gamma'_i\subset\Gamma_i$. We define~$\kappa_i(\zerovec)=1$. For a
set~$B\subseteq\Gamma_i$, let~$\extand(B)$ be the number of maximum
matchings obtained for the compatibility graph which results from
removing~$B$ from~$\Gamma_i$.
As in Section~\ref{sec:conjunction}, we will assume that
$\chi(b) = 1$ for all $b \in \boolattribs$.
%%
%\begin{lemma}
\medskip

\noindent
\textbf{Statement of Lemma~\ref{lem:and_supermodular}:}~
Consider an agent~$x_i\in\agset$ and the~$\frameworkand$ framework. 
Let $G$ denote the compatibility graph where $\kappa_i$ is the
compatibility function of $x_i$. For
any ~$B\subseteq \Gamma_i$, let $G_B$
denote the compatibility graph when $\kappa_i$ is extended by
deleting the variables in $B$.
Suppose for any ~$B\subseteq\boolattribs\setminus\Gamma_i$, $G$
and $G_B$ have the same maximum matching size
(Matching scenario~2). Then, the
function~$\extand(\cdot)$ is monotone non-decreasing and supermodular.
%\end{lemma}
%%

\medskip

\noindent
\textbf{Proof.}~
Let~$B\subset B'\subseteq\Gamma_i$. Since for any
resource~$y_j$,~$\Gamma_i\setminus B'\subseteq \Gamma_i\setminus B$, the
compatibility graph  $G_{B}$ resulting from removing~$B'$ will be a subgraph of the one resulting from removing~$B'$. 
Hence,~$\extand(B)\le\extand(B')$; that is,
$\extand(\cdot)$ is a monotone non-decreasing function.

Now, we will show that for any~$B,B'\subseteq\Gamma_i$,
~$\extand(B)+\extand(B')\le\extand(B\cup B')+\extand(B\cap B')$.
As in Theorem~\ref{thm:or_greedy}, since the maximum matching size does not
increase with the addition of attribute values, the maximum matchings in
the original compatibility graph are also maximum matchings in the new
graph. Also, we will be using the notation~$\miold$ and~$\misize{B}$
defined in~Theorem~\ref{thm:or_greedy}.  Suppose~$y_j$ is an incompatible
resource which becomes compatible on deleting~$B\cup B'$. This means
that~$\Gamma_i\nsubseteq B_j$, but~$\Gamma_i\setminus(B\cup B')\nsubseteq
B_j$. We will define four classes (induced by~$B$ and~$B'$) into which such
resources can be partitioned.
%%
\begin{align}%\label{eqn:classes_two}
y_j\in\left\{
\begin{array}{ll}
C_1, & \text{if $\Gamma_i\subseteq B$ and $\Gamma_i\subseteq B'$}, \\ 
C_2, & \text{if $\Gamma_i\subseteq B$ and $\Gamma_i \nsubseteq B'$}, \\
C_3, & \text{if $\Gamma_i\nsubseteq B$ and $\Gamma_i \subseteq B'$}, \\
C_4, & \text{if $\Gamma_i\nsubseteq B$ and $\Gamma_i \nsubseteq B'$}
\end{array}
\right.
\end{align}
%%
Let~$m_\ell$ denote the number of new maximum matchings obtained by adding
all edges~$(x_i,y_j)$,~$y_j\in C_\ell$ to the compatibility graph.  Note
that~$\extand(B\cap B')$ corresponds to maximum matchings obtained from
adding all resources belonging to~$C_1$, and therefore,~$\extand(B\cap
B')=\miold+m_1$. The quantity~$\extand(B)$ corresponds to maximum matchings
resulting from adding resources from~$C_1$ and~$C_2$, and
therefore,~$\extand(B)=\miold+m_1+m_2$.
Similarly,~$\extand(B')=\miold+m_1+m_3$. Finally,~$\extand(B\cup
B')=\miold+m_1+m_2+m_3+m_4$.
Clearly,~$\extand(B)+\extand(B')\le\extand(B\cup B')+\extand(B\cap B')$.
\QED

In Algorithm~\ref{alg:and_greedy}, we describe a greedy algorithm for this
problem, which is similar to Algorithm~\ref{alg:or_greedy}.
However, the performance guarantee result is different since
the function considered is supermodular.
%%
\begin{algorithm}[!htb]
\caption{Approximation algorithm for~$\frameworkand$\label{alg:and_greedy}}
\DontPrintSemicolon
\BlankLine
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{
Resources~$\rset$, agents~$\agset$, variables for attribute values~$\boolattribs$,
compatibility graph~$G(V_{\sagset},V_{\srset},E)$ and advice
framework~$\frameworkand(\forbidden,\attvec,\compatibilityset,\kappa_i,\chi)$
with~$\chi(b) = 1$ for all $b \in \boolattribs$.
Budget~$\beta$.
}
\Output{Extension~$\kappa^g_i$ of~$\kappa_i$
with~$\cost(\kappa^g_i)\le\beta$}
%%
\tcp{Matching scenario 1}
Let~$M(G)$ be the size of a maximum matching in~$G$.
\For{$y_j\in\rset\setminus\forbidden$ s.t. $y_j$ not compatible with~$x_i$}{
    Let~$G_j=G(V_{\sagset},V_{\srset},E\cup\{x_i,y_j\})$.\;
    %%Let~$c'=\sum_{b\in \Gamma_i\setminus B_j}\chi(b)$.\;
    %%\If{$M(G_j)>M(G)$ and $c'\le\beta$}{
    \If{$M(G_j)>M(G)$}{
        \If{$|\Gamma_i\setminus B_j|\le\beta$}{
        \Return~$\kappa^g_i=\And_{b\in \Gamma_i\setminus B_j}b$.\;
        }
        \Else{
            Set $\forbidden\leftarrow\forbidden\cup\{y_j\}$.
        }
    }
}
\tcp{Matching scenario 2}
Let $\Gamma=\Gamma_i$,~$\cost^g=0$.\;
%%Let~$B=\{b\in \Gamma\mid c_b\le\beta\}$.\;
%%\While{$B\ne\varnothing$}{
\While{$\cost^g<\beta$}{
    \For{$b\in \Gamma$}{
        Let~$\kappa^b_i=\And_{b'\in \Gamma\setminus\{b\}}b'$.
        Compute~$\benefit(\kappa_i^b)$.\;
        %%Let~$\kappa_i^b$ denote conjunction of literals in~$\Gamma\setminus\{b\}$.\;
    }
    %%Let~$b^*=\argmax_{b\in B}\frac{\benefit(\kappa_i^b)}{\cost(\kappa_i^b)}$.\;
    Let~$b^*=\argmax_{b\in B}\benefit(\kappa_i^b)$.\;
    Set~$\Gamma\leftarrow\Gamma\setminus\{b^*\}$
    and~$\cost^g\leftarrow\cost^g+1$.\;
    %%Let~$B=\{b\in \Gamma\mid c_b\le\beta-\cost^g\}$.\;
}
Set~$\kappa_i^g$ as conjunction of literals in~$\Gamma$.\;
\Return $\kappa^g_i$
%%
\end{algorithm}
%%
To analyze the performance guarantee provided by 
Algorithm~\ref{alg:and_greedy}, we need to define the quantity \emph{submodularity ratio}~\cite{das2011submodular}.
It should be noted that the submodularity ratio is a non-negative
number whose value is at most 1.
%%
\begin{definition}[Submodularity ratio]%\label{def:subratio}
The submodularity ratio of a non-negative set function~$F(\cdot)$ defined
over a ground set~$\mathcal{V}$ is the largest scalar~$\gamma$ such that
$\forall S,T\subseteq\mathcal{V}$, $\sum_{x\in T\setminus S}
F(S\cap\{x\})-F(S)\ge \gamma(F(S\cap T)-F(S))$.
\end{definition}

\medskip

\noindent
\textbf{Statement of Theorem~\ref{thm:and_greedy}:}
Consider the \problem{} for a customer~$x_i$
under~$\frameworkand(\forbidden,\attvec,\compatibilityset,\kappa_i,\chi)$
framework where~$\chi$ is a non-zero uniform cost function.
Algorithm~\ref{alg:and_greedy} provides an extension~$\kappa^g_i$ with cost
at most~$\beta$ and guarantees an approximation ratio of~$\gamma$, the
submodularity ratio of~$\extand$, i.e.,~$\benefit(\kappa^g_i)\ge
\gamma\benefit(\kappa^*_i)$.
The algorithm uses at most $m = |\rset|$ calls to the matching
oracle. The other parts of the algorithm run in polynomial time.

\medskip

\noindent
\textbf{Proof.~}
The proof is similar to that of~Theorem~\ref{thm:or_greedy}.  There are two
parts to Algorithm~\ref{alg:and_greedy}. The first part handles Matching
scenario~1. For each incompatible resource~$y_j$, it checks whether making
it compatible increases the maximum matching size in the resulting
graph~$G_j$. If this is indeed the case, then by Part~1 of
Definition~\ref{def:matching_scenarios},~$x_i$ is matched in all maximum
matchings of~$G'$. Therefore, this is the best benefit one can obtain after
extending~$\kappa_i$. This can be realized by removing all variables
in~$\Gamma_i$. However, if the total cost exceeds~$\beta$,
this cannot be done. We place such~$y_j$ in the forbidden set. This ensures
that for any remaining~$y_j$, the maximum matching size cannot be increases
by adding it to the compatibility graph. Therefore, we have Matching
Scenario~2. For this case, by
Lemma~\ref{lem:and_supermodular},~$\extand(\cdot)$ is supermodular. It
follows by~Bian~et~al.~(\citeyear{bian2017guarantees}) that the greedy
algorithm in the second part of Algorithm~\ref{alg:and_greedy} guarantees
the~$\gamma$ approximation ratio for \problem{}. We will complete the proof
by bounding the running time.

To check for Matching scenario~1, we need to compute at most~$m$ maximum
matchings, one for each~$G_j$. As explained in the
proof of Theorem~\ref{thm:or_greedy}, the time used to compute
these matchings is
$O\big(m((n+m)^{2.5})\big)$.
As before, Matching scenario~2 requires at most~$m$ calls 
to the matching oracle (by
Lemma~\ref{lem:oracle_calls}). In each iteration~$\ell$, at
most~$|\Gamma_i|-\ell$ variables will be evaluated to identify~$b^*$.
To compute~$\benefit(\kappa_i^b)$, we need to find the set of resources
that become compatible for each node (at most~$m$ operations). Once we have
this set, by Lemma~\ref{lem:oracle_calls}, the benefit can be computed.
This takes time~$O(\beta\,m|\Gamma_i|)$ assuming each variable has
unit cost. 
Thus, the algorithm uses at most $m$ calls to the matching
oracle and the running time of the other parts of the 
algorithm is $O\big(m(n+m)^{2.5} + \beta\,m|\Gamma_i|\big)$.
\QED

\subsection{Statement and Proof of Theorem~\ref{thm:threshold}}

\underline{Statement of Theorem~\ref{thm:threshold}:}
Consider the \problem{} problem for a customer~$x_i$
under the $\frameworkth(\forbidden,\attvecth,\compatth,\kappa_i,\chith)$
framework.  Algorithm~\ref{alg:thresh} provides an optimal
extension~$\kappa^*_i$ with cost at most~$\beta$ in
time~$O(\beta^\alpha\log|\boolattribs|)$.
The number of calls to the matching oracle is at most $m$.


\section{Additional Material for Section~\ref{sec:experiments}}
\label{sec:supp_experiments}

\begin{figure}[t]
\centering
\small
\includegraphics[width=.28\textwidth]{sup_figures/synthetic_random_relax_beta.png}
\caption{$\frameworkand$ average probability improvement for different $\beta$ values}
\end{figure}
%%
\subsection{More details regarding datasets}
There are two real-world datasets that we considered: The \emph{Children
Summer Vacation Activities} or \emph{Passeport
Vacances}~(\pv)~\cite{varone2019dataset} and the \emph{Course-Classroom}
(\cc) datasets.  \pv{} is based on online registration for assigning
holiday activities to children. There are two attributes -- minimum and
maximum permissible age for participation with ranges $6-15$ and~$7-16$
respectively. A child has preferences about which activity it would like to
participate with range~$0-5$. Accordingly, the compatibility function has
three attributes: minimum age, maximum age and preferences. Note that each
attribute induces a threshold function. There are three time slots for
these activities. We used one of the time slots for which the total number
of children and activities are~$694$ and~$249$ respectively.  Although the
problem of assigning classrooms to courses is quite
common~\cite{phillips2015integer}, we did not find any publicly
available dataset that could be used here. Our new classroom assignment dataset comes from a
university for the year~2018--2019\footnote{Additional information about the data set will be provided in the final version of the paper.}. 
We picked a
particular time slot (2pm--4pm) on a particular weekday for which we have~$144$ classrooms
and~$154$ courses. Each classroom has four attributes: its \emph{capacity} 
(range~$16-270$), \emph{region} to which it belongs
to~(range~$1-8$), whether it allows students with  physical disability and whether it allows students with
hearing disability; each of the last two attributes takes two values -- true or false.  For
many of the courses there were specific region preferences. Since we
couldn't find real details about people with disability, we assigned the
disability preference randomly to courses assuming that the total number of
people with disabilities is~$60$, which was the actual number for the
relevant year. 
We  also considered Erd\"{o}s-Renyi random bipartite graphs
\cite{EK-2010}
with~$5-15$ agents and~$10-15$ resources with different edge
probabilities~$p \in \{0.05,..0.5\}$
for experiments with~$\frameworkor$ and~$\frameworkand$ frameworks each
with~$10$ replicates. We also used~$40\times40$ and~$80\times40$ bipartite
graphs to evaluate the \hkuno{} algorithm.
%% %%
%% \begin{figure*}[t]
%% \centering
%% \small
%% \includegraphics[width=0.28\textwidth]{figures/theta1_change.png}
%% \includegraphics[width=0.26\textwidth]{figures/theta2_change.png}
%% \includegraphics[width=0.28\textwidth]{figures/p_change.png}
%% \includegraphics[width=0.16\textwidth]{figures/0.35_10_10_1000.png}
%% \caption{Evaluation of \rhk{} random graphs. The first three plots show how
%%     the average estimated probability~$\empprob$ compares with~$\trueprob$
%%     for $100$ random graphs of size~$10\times10$ for varying (a)~$\nhk$,
%%     (b)~$\nuno$ and random graph edge probability~$p$. The fourth plot
%%     shows variation in the Average mean square error (MSE) in a set of~$1000$ 
%%     random graphs with~$p=0.35$ for varying~$\nhk$ (y-axis) and~$\nuno$
%%     (x-axis). The lighter squares indicate greater mistakes. \label{fig:hkuno}}
%% \end{figure*}

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% We are not doing this in the AAMAS-2022 submission.
%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluating \hkuno{} algorithm}
For the \rhk{} algorithm, we used the implementation in the Python NetworkX
Package~(\citeyear{SciPyProceedings_11}) and for the ``Uno'' component of
the algorithm we used a github
implementation\footnote{https://github.com/Xunius/bipartite\textunderscore
matching} as a basis. For each graph, we calculated the empirical
probability~$\empprob$ for each node using \rhk{} with different
parameters. The results were averaged over multiple nodes and multiple
graphs and compared to the ~$\trueprob$ by using the
Uno~(\citeyear{uno1997algorithms}) algorithm. For smaller graphs, we
compared the \rhk{}$(\nhk,\nuno)$ with the true probability computed by
generating all matching using the Uno algorithm (Figure~\ref{fig:hkuno}).
The main conclusion from the figure is that with few repetitions
of~$\nhk$ and~$\nuno$, the average Mean Square Error (MSE)
quickly reduces to acceptable
values. Secondly, we note from Figure~\ref{fig:hkuno}(c) that as the graph
becomes dense and the probability of being matched increases, the error
goes down. In particular, for very sparse graphs, we need to have
relatively large~$\nhk$ values.
%%%%%%%%%%%%%%%%%%%%%%%%
\fi

\subsection{Experiments on $\frameworkor$ and $\frameworkand$ with synthetic graphs}
We experimented extensively on synthetic graphs to evaluate the greedy algorithms
developed in Algorithm~\ref{alg:or_greedy} and 
Algorithm~\ref{alg:and_greedy}.
%\footnote{Descriptions of these two algorithms are given discussed in Section~\ref{sec:sup_customer_side}
%of this Supplement.}
We used
exhaustive search to obtain a pseudo-optimal solution (since the probabilities are
only estimates) and compared it with the greedy solution. 
The~$(|\agset|, |\rset|)$ pairs considered
were~$(40,20)$ and~$(80,40)$ with 
probability~$0.2$. We considered various combinations 
of~$|\boolattribs|$ ($2-12$), number of attributes per resource~$|B_j|$ 
($1-5$), $|\Gamma_i|$ ($1-5$) and budget~$\beta$ ($1-5$). For each instance, we ran~300
experiments of finding extensions to the compatibility function. 
Interestingly, the
greedy algorithm matched the performance 
of the pseudo-optimal solution in most cases. Figure 3 demonstrates the effectiveness of $\frameworkand$ in the improvement of the probability for different $\beta$ values. 
As one would expect, the average improvement in
probability increases with the budget.
\paragraph{Evaluating \hkuno{} algorithm.}
Implementation details related to this aspect are covered in the
supplement. For each random bipartite graph, we calculated the empirical
probability~$\empprob$ for each node for various combinations of~$\nhk$
and~$\nuno$. The results averaged over multiple nodes and multiple
graphs and compared to the true $\trueprob$ values by using the
Uno~(\citeyear{uno1997algorithms}) algorithm are in Figure~\ref{fig:hkuno}.
The main conclusion from the figure is that with small values of~$\nhk$
and~$\nuno$, the average Mean Square Error (MSE) quickly reduces to
acceptable values. Secondly, we note from Figure~\ref{fig:hkuno}(c) that as
the graph becomes dense and the probability of being matched increases, the
error goes down. In particular, for very sparse graphs, we need to have
relatively large~$\nhk$ values.
%%
%% \paragraph{Experiments on $\frameworkor$ and $\frameworkand$ with synthetic
%% graphs.} We experimented extensively on synthetic graphs to evaluate the
%% greedy algorithms developed in Algorithm~\ref{alg:or_greedy} and
%% Algorithm~\ref{alg:and_greedy}\footnote{Algorithm~\ref{alg:and_greedy} is
%% discussed in the Supplement.} We used exhaustive search to obtain a
%% pseudo-optimal solution (since the probabilities are only estimates) and
%% compared it with the greedy solution. The details of the graphs and the
%% matching framework's parameters are in the supplement. Interestingly, the
%% greedy algorithm matched the performance of the pseudo-optimal solution in
%% most cases.


\noindent
%We develop rigorous combinatorial formulations using
%submodular and supermodular functions.
\underline{2. Estimating the probability of an agent being
assigned a}\newline
\underline{resource:}~ 
%\textcolor{red}{(Will we have this result in the paper?)}
Given an agent, the goal here is to find the probability
that a maximum matching chosen uniformly randomly from the set of
all maximum matchings includes that agent.
%\textcolor{red}{(Ravi: Check the next statement about complexity.)}
This problem is closely related to a computationally intractable (technically, \cnump-hard) problem, namely counting 
the number of maximum matchings in bipartite graphs 
\cite{miklos2020counting,Jerrum-1987}.
So, we develop a heuristic for this estimation using
the Hopcroft-Karp maximum matching algorithm 
\cite{Hopcroft-Karp-1973} and Uno's
algorithm for enumerating maximum matchings \cite{uno1997algorithms}.
We present experimental results for our heuristic.

the event that
resources in~$\rset_\ell$ become compatible upon relaxing~$A$. Let~$\rcoll$
denote that set of 


$\kappa'_i(\attvec(y_a))=
\kappa'_i(\attvec(y_b))$ for every
extension~$\kappa'_i$ of~$\kappa_i$. Then, to evaluate any extension
of~$\kappa_i$, it suffices to know the number of new maximum matchings
obtained by adding exactly~$\rset_l$ to the original compatibility graph,
for all~$\ell=1,2,\ldots,\eta$. Further, let~$\distattset=\{A_i\mid \forall
y_i\in \rset\}$ be the collection of distinct attribute value sets among
the resources in~$\rset$.  Then,~$\eta\le|\distattset|\le m$, where~$m$ is
the number of resources.
%\end{lemma}
\noindent
\textbf{Proof.~} For any set of new resources~$Y\subseteq\rset$ added to
the compatibility graph due to the extension of $\kappa_i$ to
$\kappa'_i$, let~$\nmsize{Y}$ denote the number of new maximum
matchings resulting from this addition. By Lemma~\ref{lem:matching_size},
each such matching has exactly one new resource matched to~$x_i$. Hence,
$\benefit(\kappa'_i)=\sum_{y\in Y}\nmsize{\{y\}}$.
Since for any~$y,y'\in\rset_\ell$,~$y\in Y$ implies~$y'\in Y$, it follows
that~$\benefit(\kappa'_i)=\sum_\ell\nmsize{\rset_\ell}$. Therefore, it is
enough to compute the number of new matchings resulting from
adding exactly~$\rset_{\ell}$ to the compatibility graph for
all~$\ell=1,\ldots,\eta$.

Next, we note that by the definition of the compatibility function, for
any~$y_j\in \rset$, the value~$\kappa'_i(A_j)$ depends
on~$\Gamma'_i\cap\{b_a\mid a\in A_j\}$, where~$\Gamma'_i$ is the set of
Boolean variables appearing in the formula of~$\kappa'_i$. Therefore, for
any~$y_{j'}$,~$\kappa'_i(\attvec(y_{j'})) = \kappa'_i(\attvec(y_j))$.
Hence,~$\eta\le|\distattset|$.
\QED
The third type of framework is the \emph{conjunction of threshold
functions}. Let $\mathbb{R}$ denote the set of real numbers.
A \textbf{threshold} function 
$g_{\tau} \,:\, \mathbb{R} \rightarrow \{0,1\}$
is characterized by a non-negative threshold value $\tau$; for any
$t \in \mathbb{R}$,
$g_{\tau}(t) = 1$ if $t \geq \tau$ and 0 otherwise.
%for consists of a non-negative real-value
%called threshold. The input to the function is again a non-negative
%real-value. The function returns true iff the input is greater than or
%equal to the threshold. 
In our setting, we assume that the variables of
every attribute have a natural ordering, say~$b_1<b_2<\cdots$. 
For every resource~$y_j$, the attribute function satisfies the following
condition:~$b_k=1$ implies
that~$b_{k-1}=1$, for all $k \geq 2$.
We refer to this attribute function as~$\attvecth$.  For
agent~$x_i$,~$b_k\in \Gamma_i$ implies that~$b_{k-1}\in \Gamma_i$. 
We refer
to this class of functions as~$\compatth$.  
For~$y_j$,
let~$b_{\min}^j=\argmax_{b_k} b_k=1$ and let threshold of~$x_i$
be~$\tau_i=\argmin_{b_k} b_k\in \Gamma_i$. 
It is easy to see that the clause
is true iff~$\tau_i\ge b_{\min}^j$. Finally, we define a monotone cost
function~$\chith(b_k)$ as the cost of changing the threshold to~$b_k$. It has the following property, $\forall b,b'\in \boolattribs$, $b<b'$
implies~$\chith(b)>\chith(b')$. 
The rationale behind this cost function is
that the more one deviates from the threshold, 
the larger is the cost. The
threshold framework comprises of these components and is denoted
by~$\frameworkth(\forbidden,\attvecth,\compatth,\kappa_i,\chith)$.


\subsection{The~$\frameworkand$ framework with uniform costs}
\label{sec:conjunction}
We have also developed an approximation algorithm similar
to Algorithm~\ref{alg:or_greedy}
for the $\frameworkand$~ framework again assuming 
uniform costs. 
The main difference is that the corresponding function
$\extand$ is supermodular.
The details of this approximation algorithm and its
performance guarantee are given in the supplement.

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%
We recall that~$x_i$ and~$y_j$ are compatible only if~$\Gamma_i\subseteq
B_j$. Therefore,~$\kappa'_i$ is an extension of~$\kappa_i$
iff~$\Gamma'_i\subset\Gamma_i$. We define~$\kappa_i(\zerovec)=1$. For a
set~$B\subseteq\Gamma_i$, let~$\extand(B)$ be the number of maximum
matchings obtained for the compatibility graph which results from
removing~$B$ from~$\Gamma_i$.
As in Section~\ref{sec:conjunction}, we will assume that
$\chi(b) = 1$ for all $b \in \boolattribs$.
%%
\begin{lemma}
\label{lem:and_supermodular}
Consider an agent~$x_i\in\agset$ and the~$\frameworkand$ framework. 
Let $G$ denote the compatibility graph where $\kappa_i$ is the
compatibility function of $x_i$. For
any ~$B\subseteq \Gamma_i$, let $G_B$
denote the compatibility graph when $\kappa_i$ is extended by
deleting the variables in $B$.
Suppose for any ~$B\subseteq\boolattribs\setminus\Gamma_i$, $G$
and $G_B$ have the same maximum matching size
(Matching scenario~2). Then, the
function~$\extand(\cdot)$ is monotone non-decreasing and supermodular.
\end{lemma}
%%
\noindent
\textbf{Proof.}~
Let~$B\subset B'\subseteq\Gamma_i$. Since for any
resource~$y_j$,~$\Gamma_i\setminus B'\subseteq \Gamma_i\setminus B$, the
compatibility graph  $G_{B}$ resulting from removing~$B'$ will be a subgraph of the one resulting from removing~$B'$. 
Hence,~$\extand(B)\le\extand(B')$; that is,
$\extand(\cdot)$ is a monotone non-decreasing function.

Now, we will show that for any~$B,B'\subseteq\Gamma_i$,
~$\extand(B)+\extand(B')\le\extand(B\cup B')+\extand(B\cap B')$.
As in Theorem~\ref{thm:or_greedy}, since the maximum matching size does not
increase with the addition of attribute values, the maximum matchings in
the original compatibility graph are also maximum matchings in the new
graph. Also, we will be using the notation~$\miold$ and~$\misize{B}$
defined in~Theorem~\ref{thm:or_greedy}.  Suppose~$y_j$ is an incompatible
resource which becomes compatible on deleting~$B\cup B'$. This means
that~$\Gamma_i\nsubseteq B_j$, but~$\Gamma_i\setminus(B\cup B')\nsubseteq
B_j$. We will define four classes (induced by~$B$ and~$B'$) into which such
resources can be partitioned.
%%
\begin{align}\label{eqn:classes_two}
y_j\in\left\{
\begin{array}{ll}
C_1, & \text{if $\Gamma_i\subseteq B$ and $\Gamma_i\subseteq B'$}, \\ 
C_2, & \text{if $\Gamma_i\subseteq B$ and $\Gamma_i \nsubseteq B'$}, \\
C_3, & \text{if $\Gamma_i\nsubseteq B$ and $\Gamma_i \subseteq B'$}, \\
C_4, & \text{if $\Gamma_i\nsubseteq B$ and $\Gamma_i \nsubseteq B'$}
\end{array}
\right.
\end{align}
%%
Let~$m_\ell$ denote the number of new maximum matchings obtained by adding
all edges~$(x_i,y_j)$,~$y_j\in C_\ell$ to the compatibility graph.  Note
that~$\extand(B\cap B')$ corresponds to maximum matchings obtained from
adding all resources belonging to~$C_1$, and therefore,~$\extand(B\cap
B')=\miold+m_1$. The quantity~$\extand(B)$ corresponds to maximum matchings
resulting from adding resources from~$C_1$ and~$C_2$, and
therefore,~$\extand(B)=\miold+m_1+m_2$.
Similarly,~$\extand(B')=\miold+m_1+m_3$. Finally,~$\extand(B\cup
B')=\miold+m_1+m_2+m_3+m_4$.
Clearly,~$\extand(B)+\extand(B')\le\extand(B\cup B')+\extand(B\cap B')$.
\QED

In Algorithm~\ref{alg:and_greedy}, we describe a greedy algorithm for this
problem, which is similar to Algorithm~\ref{alg:or_greedy}.
However, the performance guarantee result is different since
the function considered is supermodular.
%%
\begin{algorithm}[!htb]
\caption{Approximation algorithm for~$\frameworkand$\label{alg:and_greedy}}
\DontPrintSemicolon
\BlankLine
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{
Resources~$\rset$, agents~$\agset$, variables for attribute values~$\boolattribs$,
compatibility graph~$G(V_{\sagset},V_{\srset},E)$ and advice
framework~$\frameworkand(\forbidden,\attvec,\compatibilityset,\kappa_i,\chi)$
with~$\chi(b) = 1$ for all $b \in \boolattribs$.
Budget~$\beta$.
}
\Output{Extension~$\kappa^g_i$ of~$\kappa_i$
with~$\cost(\kappa^g_i)\le\beta$}
%%
\tcp{Matching scenario 1}
Let~$M(G)$ be the size of a maximum matching in~$G$.
\For{$y_j\in\rset\setminus\forbidden$ s.t. $y_j$ not compatible with~$x_i$}{
    Let~$G_j=G(V_{\sagset},V_{\srset},E\cup\{x_i,y_j\})$.\;
    %%Let~$c'=\sum_{b\in \Gamma_i\setminus B_j}\chi(b)$.\;
    %%\If{$M(G_j)>M(G)$ and $c'\le\beta$}{
    \If{$M(G_j)>M(G)$}{
        \If{$|\Gamma_i\setminus B_j|\le\beta$}{
        \Return~$\kappa^g_i=\And_{b\in \Gamma_i\setminus B_j}b$.\;
        }
        \Else{
            Set $\forbidden\leftarrow\forbidden\cup\{y_j\}$.
        }
    }
}
\tcp{Matching scenario 2}
Let $\Gamma=\Gamma_i$,~$\cost^g=0$.\;
%%Let~$B=\{b\in \Gamma\mid c_b\le\beta\}$.\;
%%\While{$B\ne\varnothing$}{
\While{$\cost^g<\beta$}{
    \For{$b\in \Gamma$}{
        Let~$\kappa^b_i=\And_{b'\in \Gamma\setminus\{b\}}b'$.
        Compute~$\benefit(\kappa_i^b)$.\;
        %%Let~$\kappa_i^b$ denote conjunction of literals in~$\Gamma\setminus\{b\}$.\;
    }
    %%Let~$b^*=\argmax_{b\in B}\frac{\benefit(\kappa_i^b)}{\cost(\kappa_i^b)}$.\;
    Let~$b^*=\argmax_{b\in B}\benefit(\kappa_i^b)$.\;
    Set~$\Gamma\leftarrow\Gamma\setminus\{b^*\}$
    and~$\cost^g\leftarrow\cost^g+1$.\;
    %%Let~$B=\{b\in \Gamma\mid c_b\le\beta-\cost^g\}$.\;
}
Set~$\kappa_i^g$ as conjunction of literals in~$\Gamma$.\;
\Return $\kappa^g_i$
%%
\end{algorithm}
%%
To analyze the performance guarantee provided by 
Algorithm~\ref{alg:and_greedy}, we need to define the quantity \emph{submodularity ratio}~\cite{das2011submodular}.
It should be noted that the submodularity ratio is a non-negative
number whose value is at most 1.
%%
\begin{definition}[Submodularity ratio]\label{def:subratio}
The submodularity ratio of a non-negative set function~$F(\cdot)$ defined
over a ground set~$\mathcal{V}$ is the largest scalar~$\gamma$ such that
$\forall S,T\subseteq\mathcal{V}$, $\sum_{x\in T\setminus S}
F(S\cap\{x\})-F(S)\ge \gamma(F(S\cap T)-F(S))$.
\end{definition}

\begin{theorem}\label{thm:and_greedy}
Consider the \problem{} for a customer~$x_i$
under~$\frameworkand(\forbidden,\attvec,\compatibilityset,\kappa_i,\chi)$
framework where~$\chi$ is a non-zero uniform cost function.
Algorithm~\ref{alg:and_greedy} provides an extension~$\kappa^g_i$ with cost
at most~$\beta$ and guarantees an approximation ratio of~$\gamma$, the
submodularity ratio of~$\extand$, i.e.,~$\benefit(\kappa^g_i)\ge
\gamma\benefit(\kappa^*_i)$.
The algorithm uses at most $m = |\rset|$ calls to the matching
oracle. The other parts of the algorithm run in polynomial time.
\end{theorem}
\noindent
\textbf{Proof.~}
The proof is similar to that of~Theorem~\ref{thm:or_greedy}.  There are two
parts to Algorithm~\ref{alg:and_greedy}. The first part handles Matching
scenario~1. For each incompatible resource~$y_j$, it checks whether making
it compatible increases the maximum matching size in the resulting
graph~$G_j$. If this is indeed the case, then by Part~1 of
Definition~\ref{def:matching_scenarios},~$x_i$ is matched in all maximum
matchings of~$G'$. Therefore, this is the best benefit one can obtain after
extending~$\kappa_i$. This can be realized by removing all variables
in~$\Gamma_i$. However, if the total cost exceeds~$\beta$,
this cannot be done. We place such~$y_j$ in the forbidden set. This ensures
that for any remaining~$y_j$, the maximum matching size cannot be increases
by adding it to the compatibility graph. Therefore, we have Matching
Scenario~2. For this case, by
Lemma~\ref{lem:and_supermodular},~$\extand(\cdot)$ is supermodular. It
follows by~Bian~et~al.~(\citeyear{bian2017guarantees}) that the greedy
algorithm in the second part of Algorithm~\ref{alg:and_greedy} guarantees
the~$\gamma$ approximation ratio for \problem{}. We will complete the proof
by bounding the running time.

To check for Matching scenario~1, we need to compute at most~$m$ maximum
matchings, one for each~$G_j$. As explained in the
proof of Theorem~\ref{thm:or_greedy}, the time used to compute
these matchings is
$O\big(m((n+m)^{2.5})\big)$.
As before, Matching scenario~2 requires at most~$m$ calls 
to the matching oracle (by
Lemma~\ref{lem:oracle_calls}). In each iteration~$\ell$, at
most~$|\Gamma_i|-\ell$ variables will be evaluated to identify~$b^*$.
To compute~$\benefit(\kappa_i^b)$, we need to find the set of resources
that become compatible for each node (at most~$m$ operations). Once we have
this set, by Lemma~\ref{lem:oracle_calls}, the benefit can be computed.
This takes time~$O(\beta\,m|\Gamma_i|)$ assuming each variable has
unit cost. 
Thus, the algorithm uses at most $m$ calls to the matching
oracle and the running time of the other parts of the 
algorithm is $O\big(m(n+m)^{2.5} + \beta\,m|\Gamma_i|\big)$.
\QED
%%%%%%%%%%%%%%%%%%%%
\fi

\subsection{The threshold framework $\frameworkth$}
\label{sec:threshold}
We now describe an algorithm for finding an
optimal solution to the \problem{} problem
for the~$\frameworkth$ framework (Algorithm~\ref{alg:thresh}). Throughout,
we will assume that the costs defined by~$\chith(\cdot)$ are integer
valued. Suppose there are~$\alpha$ attributes.
Let~$\boolattribs=\biguplus_{1\le\ell\le\alpha}\boolattribs_\ell$ be a
partition of variables where each part contains variables corresponding to
values of an attribute.
We say that an $\alpha$-tuple $(\beta_1,\beta_2,\ldots,\beta_\alpha)$
of non-negative integers
is an $\alpha$-partition of the
 the budget~$\beta$ if $\sum_{\ell=1}^{\alpha} \beta_{\ell} = \beta$.
Let~$\partitionset$ denote all the $\alpha$-partitions of~$\beta$.
Algorithm~\ref{alg:thresh} exhaustively explores all possible budget
allocations to the attributes. Once the budget is allocated, the
best solution among the attribute values in each~$\boolattribs_\ell$ can be
computed using a binary search. Our solution simply sets the threshold to this attribute value.
%%
\begin{algorithm}[!htb]
\caption{Algorithm for~$\frameworkth$\label{alg:thresh}}
\DontPrintSemicolon
\BlankLine
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{
Resources~$\rset$, agents~$\agset$, attribute values~$\boolattribs$
compatibility graph~$G(V_{\sagset},V_{\srset},E)$ and advice
framework $\frameworkth(\forbidden,\attvecth,\compatth,\kappa_i,\chith)$.
Budget~$\beta$ (positive integer).
\Output{Extension~$\kappa^*_i$ of~$\kappa_i$}
}
Let~$\kappa^*_i=\kappa_i$.\;
\For{Each $(\beta_1,\beta_2,\ldots,\beta_\alpha)\in\partitionset$}{
    Let~$\kappa'_i\leftarrow\compatth$.\;
    \For{$\ell=1,2,\ldots,\alpha$}{
        $b =\argmin_{b\in\boolattribs_\ell}
        \chith(b)\le\beta_\ell$.\label{alg:threshold:min}\;
        Set threshold of~$\ell$th clause to~$b$ in~$\kappa'_i$.
    }
    \lIf{$\benefit(\kappa'_i)>\benefit(\kappa^*_i)$}{$\kappa^*_i=\kappa'_i$}
}
\Return $\kappa_i^*$
%%
\end{algorithm}
%%
\begin{theorem}\label{thm:threshold}
Consider the \problem{} problem for a customer~$x_i$
under the $\frameworkth(\forbidden,\attvecth,\compatth,\kappa_i,\chith)$
framework.  Algorithm~\ref{alg:thresh} provides an optimal
extension~$\kappa^*_i$ with cost at most~$\beta$ in
time~$O(\beta^\alpha\log|\boolattribs|)$.
The number of calls to the matching oracle is at most $m$.
\end{theorem}

\noindent
\textbf{Proof.~} See Supplement.~ $\Box$

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
First, we will show that the algorithm provides an optimal extension. Given
a budget~$\beta_\ell$ for attribute~$\ell$, we claim
that the best solution is provided
by Line~\ref{alg:threshold:min} in the algorithm. 
The proof is as follows.
For~$b'<b''$ in~$\boolattribs_\ell$, let~$\kappa'_i$ and~$\kappa"_i$ be
extensions of~$\kappa_i$ such that their threshold for the~$\ell$th
attribute is~$b'$ and~$b''$ respectively, Otherwise they are identical.
Since~$b'<b''$, by definition of the threshold framework, for
any~$y_j$,~$\kappa''_i(\attvec(y_j))=1$ implies 
that~$\kappa'_i(\attvec(y_j))=1$.
Hence,~$\benefit(\kappa'_i(y_j))\ge\benefit(\kappa''_i(y_j))$.
Next, we note that every optimal solution~$\kappa^*_i$ 
can be associated with a 
$\alpha$-partition~$(\beta^*_1,\beta^*_2,\ldots,\beta^*_\ell)$. This can be
obtained as follows: For each attribute~$\ell$, we identify the new
threshold~$b^*_\ell$ if it exists, and set~$\beta^*_\ell$
to~$\chith(b^*_\ell)$. If~$\sum_\ell\beta^*_\ell<\beta$, then we can
increase say~$\beta^*_1$ by an amount such that the sum equals~$\beta$.
Since this $\alpha$-partition is among the solutions explored by the
algorithm, it is clear that~$\kappa^*_i$ is an optimal solution.

Now we will bound the time complexity of the algorithm. Firstly, we note
that the number of $\alpha$-partitions of~$\beta$ is
$O(\beta^\alpha)$, and can be enumerated in as much time. Secondly, given
a budget~$\beta_\ell$ for clause~$\ell$, Line~\ref{alg:threshold:min} can be
computed in~$O(\log|\boolattribs_\ell|)$ time. This is because, for
every~$b'<b''$,~$\chith(b')\ge\chith(b'')$, and therefore, the best solution
can be computed using a binary search given the natural ordering of the
variables in~$\boolattribs_\ell$.
As before, by Lemma~\ref{lem:oracle_calls}, the number
of calls to the matching oracle is at most $m$.
\QED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi



For each type of advice framework introduced in
Section~\ref{sec:definitions}, we will now describe algorithms for
generating advice and provide performance guarantees.
\noindent

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
There are two parts to Algorithm~\ref{alg:or_greedy}. The first part
handles Matching scenario~1. For each incompatible resource~$y_j$, it
checks whether making it compatible increases the maximum matching size in
the resulting graph~$G_j$. If this is indeed the case, then by Part~1 of
Definition~\ref{def:matching_scenarios},~$x_i$ is matched in all maximum
matchings of~$G'$. Therefore, this is the best benefit one can obtain after
extending~$\kappa_i$, which can be realized by adding any variable
from~$B_j$ to~$\Gamma_i$. 
%% If not, then, we will make
%% all~$y_j$ such that~$M(G_j)>M(G)$ forbidden. This will ensure that the
%%maximum matching size never increases. 
Otherwise, we have Matching scenario~$2$. For this case, by
Lemma~\ref{lem:or_submodular},~$\extor(\cdot)$ is submodular. It follows from
the analysis in 
Nemhauser~et.~al.~(\citeyear{nemhauser1978analysis}) that
Algorithm~\ref{alg:or_greedy} provides stated approximation ratio
for \problem{}. We will complete the proof by bounding the 
number of calls to the matching oracle and the time for the
other steps of the algorithm.

To check for Matching scenario~1, we need to compute at most~$m$ maximum
matchings, one for each~$G_j$. Since a maximum matching in
a bipartite graph with $q$ nodes can be computed in $O(q^{2.5})$ time
\cite{Hopcroft-Karp-1973}, the time used for computing the matchings is
$O\big(m((n+m)^{2.5})\big)$
computations. Matching scenario~2 requires at most~$m$ calls to the oracle
that computes number of maximum matchings (by
Lemma~\ref{lem:oracle_calls}). In each iteration~$\ell$, at
most~$|\boolattribs|-\ell$ variables will be evaluated to identify~$b^*$.
To compute~$\benefit(\kappa_i^b)$, we need to find the set of resources
that become compatible for each node; this can be done in $O(m)$ time. 
Once we have
this set, by Lemma~\ref{lem:oracle_calls}, the benefit can be computed
in time~$O(\beta\,m|\boolattribs|)$ since each variable has
unit cost. Hence, the algorithm uses at most $m$ calls to the matching
oracle and the other parts of the algorithm run in time
$O\big(m(n+m)^{2.5} + \beta\,m|\boolattribs|\big)$ time.
\QED
%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi
    %% Let~$b^*=\argmax_{b\in B}\frac{\benefit(\kappa_i^b)}{\cost(\kappa_i^b)}$.\;
    Let~$b^*=\argmax_{b\in B}\benefit(\kappa_i^b)$.\;
    Set~$\Gamma\leftarrow\Gamma\cup\{b^*\}$
    %and~$\cost^g\leftarrow\cost^g+c_{b^*}$.\;
    and~$\cost^g\leftarrow\cost^g+1$.\;
    %%Let~$B=\{b\in \boolattribs\setminus\Gamma\mid c_b\le\beta-\cost^g\}$.\;
%%
\tcp{Matching scenario 1}
Let~$M(G)$ be the size of a maximum matching in~$G$.
\For{$y_j\in\rset\setminus\forbidden$ s.t. $y_j$ not compatible with~$x_i$}{
    Let~$G_j=G(V_{\sagset},V_{\srset},E\cup\{x_i,y_j\})$.\;
    \If{$M(G_j)>M(G)$}{
        \Return~$\kappa^g_i=\Or_{b\in \Gamma_i\cup \{b\}}b$.\;
    }
}
Since the maximum matching size does not increase with the addition of
attribute values, any maximum matching in $G_B$
is also a maximum matchings in $G_{B'}$. Let~$\miold$ denote the number
of maximum matchings in $G$. For any
set~$B\subseteq\boolattribs\setminus \Gamma_i$, let~$\misize{B}$ denote the
number of new maximum matchings in $G_B$.

%% Since~$\extor(B)=\miold + \misize{B}$ for any~$B$, to prove
%% that~$\extor(\cdot)$ is submodular, it is enough to show
%% that~$\misize{B}+\misize{B'}\ge\misize{B\cup B'}+\misize{B\cap B'}$.
number of maximum matchings
Let~$B\subset B'\subseteq\boolattribs\setminus\Gamma_i$. Since for any
resource~$y_j$,~$B_j\cap (\Gamma_i\cup B)\subseteq B_j\cap (\Gamma_i\cup
B')$, the  graph $G_B$ will be a subgraph
of $G_{B'}$.  Hence,~$\extor(B)\le\extor(B')$;
in other words, $\extor(\cdot)$ is a monotone non-decreasing function.

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For any set of new resources~$Y\subseteq\rset$ added to
the compatibility graph due to the extension of $\kappa_i$ to
$\kappa'_i$, let~$\nmsize{Y}$ denote the number of new maximum
matchings resulting from this addition. By Lemma~\ref{lem:matching_size},
each such matching has exactly one new resource matched to~$x_i$. Hence,
$\benefit(\kappa'_i)=\sum_{y\in Y}\nmsize{\{y\}}$.
Since for any~$y,y'\in\rset_\ell$,~$y\in Y$ implies~$y'\in Y$, it follows
that~$\benefit(\kappa'_i)=\sum_\ell\nmsize{\rset_\ell}$. Therefore, it is
enough to compute the number of new matchings resulting from
adding exactly~$\rset_{\ell}$ to the compatibility graph for
all~$\ell=1,\ldots,\eta$.

Next, we note that by the definition of the compatibility function, for
any~$y_j\in \rset$, the value~$\kappa'_i(A_j)$ depends
on~$\Gamma'_i\cap\{b_a\mid a\in A_j\}$, where~$\Gamma'_i$ is the set of
Boolean variables appearing in the formula of~$\kappa'_i$. Therefore, for
any~$y_{j'}$,~$\kappa'_i(\attvec(y_{j'})) = \kappa'_i(\attvec(y_j))$.
Hence,~$\eta\le|\distattset|$.
\QED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{example}\label{ex:counting}
\smallskip
\noindent
\textbf{Example 2:}~
Consider a scenario where the compatibility functions belong to the class
$\compatand$ of conjunction of variables. Let $y_1$, $y_2$, $y_3$ and
$y_4$ be four resources with the following 
attribute values: $A_1=\{a1,a2,a4\}$, $A_2=\{a1,a2\}$, $A_3=\{a3,a4\}$,
$A_4=\{a3,a4\}$. For agent~$x_i$, let~$\kappa_i= (b_{a3}\And b_{a5})$. None
of the above resources is compatible with~$x_i$.  Any extension
of~$\kappa_i$ corresponds to removing one or both of the variables 
in $\kappa_i$.
For each resource $y_j$, let $B_j$ denote the set of Boolean
variables corresponding to the attribute value set $A_j$, $1 \leq j \leq 4$.
Thus, for any two resources~$y_j$ and~$y_{j'}$,
if~$\Gamma_i\setminus B_j=\Gamma_i\setminus B_{j'}$, then, for any
extension~$\kappa'_i$,~$\kappa'_i(\attvec(y_j)) =\kappa'_i(\attvec(y_{j'}))$. 
For example,~$y_1$ and~$y_2$ belong to the same class as both~$a3$ and~$a5$
need to be removed for them to be compatible with~$x_i$, while~$y_3$
and~$y_4$ will become compatible with $x_i$ if~$b_{a5}$ is removed from $\kappa_i$.
%\end{example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi
\subsection{Statement and Proof of Lemma~\ref{lem:matching_size}}

\underline{Statement  of Lemma~\ref{lem:matching_size}:}~
For an agent~$x_i\in \agset$, let~$\kappa_i$ and~$\kappa'_i$ denote the
compatibility function and an extension of it respectively. 
Let $G$ and $G'$ denote respectively the original 
compatibility graph (where $x_i$'s compatibility function is 
$\kappa_i$) and the one where agent $x_i$'s preference is 
$\kappa'_i$.
%We have the following observations.
\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]
\item Any maximum matching in $G'$ that was not 
a maximum matching in $G$ matches agent $x_i$ to a new resource.
\item The size of any maximum matching in $G'$
is at most one more than that of $G$.
\end{enumerate}

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Since only the compatibility function of~$x_i$ is being extended, every new
edge added to $G$ to produce $G'$ must be incident with~$x_i$. 
It can be seen that every maximum matching in $G'$ that is not a maximum matching
in $G$ must use one of the new edges added to $G$. 
Since each such edge is incident with $x_i$, the statement
of Part~1 holds. 

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Suppose
a new maximum matching was obtained upon removing restrictions in~$A$ such
that~$x_i$ was not matched in it. Then, all the edges in the matching are
edges that existed previously in the compatibility graph. Since adding
edges to the compatibility graph only increases the size of the maximum
matching, this matching is not only a matching in the original
compatibility graph, but also a maximum matching. This contradicts the
assumption that it is a new matching. Hence, we have proved Statement~1.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

Now consider Part~2. Let $\ell$ and $\ell'$ denote the sizes of maximum 
matchings in $G$ and $G'$ respectively.
For the sake of contradiction, suppose $\ell' \geq \ell+2$.
Then, there is a maximum matching $M'$ in $G'$ that is not a maximum matching
in $G$.  By Part~1, $M'$ must contain an edge $\{x_i, y_j\}$ incident with $x_i$.
Let $M$ denote the matching obtained by deleting the edge $\{x_i, y_j\}$
from $M'$.
Now, note that every edge in $M$ is also an edge in $G$; in other words,
$M$ is a matching in $G$ with at least $\ell+1$ edges.
This contradicts the assumption that the size of any maximum
matching in $G$ is $\ell$, and Part~2 follows.
\QED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi
\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Suppose
a new maximum matching was obtained upon removing restrictions in~$A$ such
that~$x_i$ was not matched in it. Then, all the edges in the matching are
edges that existed previously in the compatibility graph. Since adding
edges to the compatibility graph only increases the size of the maximum
matching, this matching is not only a matching in the original
compatibility graph, but also a maximum matching. This contradicts the
assumption that it is a new matching. Hence, we have proved Statement~1.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
which is defined as follows: given a universal set
$U = \{u_1, u_2, \ldots, u_r\}$,
a family $F = \{F_1, F_2, \ldots, F_m\}$, where $F_j \subseteq U$,
$1 \leq j \leq m$, and integers $q$ and $t$, is there a subfamily $F'$ of $F$
such that $|F'| \leq q$ and the union of the sets in $F'$ has
at least $t$ elements?
The \maxcover{} problem is known to be \cnp-complete \cite{GareyJohnson79}.
The details of the reduction are given in the supplement. $\Box$



Let $I$ denote an instance of \maxcover{} specified using the
parameters $U$, $F$, $q$ and $t$.
From $I$, we construct an instance $I'$ of \dproblem{}
as follows.

\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]
\item The agent set \agset{} = $\{x_0, x_1, x_2, \ldots, x_{r}\}$ has
$r+1$ agents while the resource set \rset{} =
$\{y_1, y_2, \ldots, y_{r}\}$ has $r$ resources.
(Recall that $r$ = $|U|$.)
The set \rset{} is in one-to-one correspondence with $U$.

\item Initially, the compatibility graph $G_0(\agset, \rset)$ has the $r$
edges given by $\{x_i, y_i\}$, $1 \leq i \leq r$. These edges form
a maximum matching of size $r$ in $G_0$.
(Thus, the number of maximum matchings in $G_0$ is 1.)

\item The compatibility function $\kappa_0$ associated with agent $x_0$
is an empty disjunction; thus, initially, no edge is incident on $x_0$.
In other words, the probability that a maximum matching in $G_0$
includes $x_0$ is zero.

\item The set $B = \{b_1, b_2, \ldots, b_m\}$ of
of Boolean variables that can be added to $\kappa_0$ is
in one-to-one correspondence with
the family $F = \{F_1, F_2, \ldots, F_m\}$.
The benefit associated with adding each of these
variables is chosen as follows.
Suppose $F_i = \{u_{i_1}, u_{i_2}, \ldots, u_{i_{\ell}}\}$, where
$\ell = |F_i|$. Then, adding the variable $b_i$ to $\kappa_0$
inserts the $\ell$ edges $\{x_0, y_{i_j}\}$, $1 \leq j \leq \ell$,
to the graph $G_0$.
(Thus, we can think of adding $b_i$ to $\kappa_0$ as adding
the edges from $x_0$ to the nodes in \rset{} corresponding to the elements of $F_i$.)
Note that when these edges are added to $G_0$, the size of the maximum matching remains $r$. However, the number of maximum matchings increases to $|F_i|+1$, and $|F_i|$ of these maximum matchings include $x_0$.
Thus, the benefit of adding $b_i$ to $\kappa_0$ is 
$|F_i|$, $1 \leq i \leq m$.

\item The cost of adding each Boolean variable $b_i$ to 
$\kappa_0$ is set to 1.
The budget $\beta$ is set to $q$, the budget on the number of sets
in the \maxcover{} instance.
The required benefit \xbenefit{} of $x_0$ is set to 
$t$, where $t$ is the
coverage requirement in the \maxcover{} instance.
\end{enumerate}
This completes the construction of the instance $I'$ of \dproblem.
It is easy to see that the construction can be carried out
in polynomial time.
We now show that there is a solution to the \dproblem{} instance $I'$
iff there is a solution to the \maxcover{} instance $I$.

\noindent
\textbf{Part 1:}~ Suppose the \maxcover{} instance $I$ has a solution.
Without loss of generality, we can assume that the solution $F'$ is given by
$F' = \{F_1, F_2, \ldots, F_q\}$ and that the sets in $F'$
cover $t' \geq t$ elements of $U$.
Consider the relaxation of the compatibility function $k_0$ (which is
an empty disjunction) to the function $k^*_0$ =
$(b_1 \vee b_2 \vee \cdots \vee b_q)$, which is obtained by adding the
Boolean variables corresponding to the sets in $F'$.
The cost of adding these variables is $q = \beta$.
Since the sets in $F'$ cover $t' \geq t$ elements of $U$,
by our construction, the function $k^*_0$ adds at least $t'$
edges to node $x_0$.
However, the maximum matching in the resulting graph remains $r$.
Thus, in the new compatibility graph obtained from $\kappa^*_0$,
the number of maximum matchings of size $r$ is $t'+1$ and $t'$
of these matchings contain $x_0$.
Thus, the benefit of $x_0$ due to the function $\kappa^*_0$ is
$t' \geq t$.  Thus, the \dproblem{} instance $I'$
has a solution.

\noindent
\textbf{Part 2:}~ Suppose the \dproblem{} instance $I'$ has a solution.
Without loss of generality, we may assume that the new compatibility
function $\kappa^*_0 = (b_1 \vee b_2 \vee \cdots \vee b_q)$.
Further, the benefit of $x_0$ due to this solution is at least $t$.
By our construction, it can be seen that the compatibility function
$\kappa^*_0$ must add at least $t$ edges to $x_0$.
Now, consider the subfamily $F' = \{F_1, F_2, \ldots, F_q\}$.
Each Boolean variable $b_i$ in $\kappa^*_0$ adds the edges corresponding
to the elements in $F_i$, $1 \leq i \leq q$.
Since $\kappa^*_0$ causes at least $t$ edges to be added to $x_0$,
it follows that the union of the sets in $F'$ covers at least
$t$ elements of $U$.
Thus, $F'$ is a solution to the \maxcover{} instance $I$, and
this completes our proof of Theorem~\ref{thm:or_hardness}. \QED
%%%%%%%%%%%%%%%%%%%%%
\fi

\medskip

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%
Our next result shows that the above hardness result holds for single
conjunctions as well.

\begin{theorem}\label{thm:and_hardness}
\dproblem{} is \cnp-hard when the function $\kappa_i$
is a conjunction of variables and the class \compatibilityset{} is
also a conjunction.
\end{theorem}

\noindent
\textbf{Proof:}~ See supplement. $\Box$
%%%%%%%%%%%%%%%%%%%%%%
\fi

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%
Since the proof is similar to that of
Theorem~\ref{thm:or_hardness}, we will only present the necessary
modifications to the above proof.

\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]
\item The initial compatibility function $\kappa_0$ for agent $x_0$ is
$(b_1 \wedge b_2 \wedge \cdots \wedge b_m)$, that is,
the conjunction of all the Boolean variables corresponding
the set family $F$. (By our convention, this function $\kappa_0$
ensures that in $G_0$, no edges are incident on $x_0$.)

\item Deleting the variable $b_i$ from $\kappa_0$ adds
between $x_0$ and the nodes in \rset{} corresponding to the elements of $F_i$.
The cost of deleting each variable from $\kappa_0$ is set to 1.

\item If the subfamily $F' = \{F_1, F_2, \ldots, F_q\}$ is a
solution to the \maxcover{} instance, then a solution to the
\dproblem{} is $(b_{q+1} \wedge b_{q+2} \wedge \cdots \wedge b_m)$
and vice versa. \QED
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%
\fi

\iffalse
%%%%%%%%%%%%%%%%%% Old hardndess result -- has a bug %%%%%%%%%%%%
Given a bipartite graph~$G$ and vertex~$v$, and a matching sampled
uniformly from the space of it's maximum matchings, we would like to
compute the probability~$p_v(G)$ that~$v$ is in that matching. It is not
possible to prove this by reduction from the problem of counting the
perfect matchings in a bipartite graph (which is \#P-hard) since in that
case,~$p_v(G)=1$. We believe that this problem is also \#P-hard. Recently,
it has been shown in an unpublished work that counting the number of
maximum matchings in a planar bipartite graph is
\#P-hard~\cite{miklos2020counting}.  We will now show that our problem is
at least as hard as counting maximum matchings in a bipartite graph.
%%
\begin{theorem}\label{thm:sharpP}
Given an arbitrary bipartite graph~$G$, computing the probability of
a node being present in a matching sampled uniformly from the set of
maximum matchings of the graph is at least as hard as computing the number
of maximum matchings in~$G$.
\end{theorem}
%%
\noindent
\textbf{Proof.~}
We prove this theorem by a reduction from the problem of counting maximum
matchings in a bipartite graph. The proof is by induction. We will start
with a maximum matching of~$G_0$ of~$G$. In every iteration~$i$, we will
add one new edge~$e_i\in E(G)\setminus E(G_i)$. Let~$\omega_i$ denote the
number of maximum matchings in~$G_i$. For a vertex~$v$, let~$\omega_i^v$
denote the number of those maximum matchings in which~$v$ is matched.
Let~$\alpha_i^v$ denote the number of new maximum matchings resulting from
adding edge~$e_i$ to~$G_{i-1}$. We will show that, given a polynomial-time
algorithm to compute~$p_v(G_i)$,~$\omega_i$ can be computed in
polynomial-time as well.

The base case corresponds to~$G_0$. Since~$G_0$ corresponds to a maximum
matching of~$G$,~$p_v(G_0)=1$ if~$v$ is matched, else~$0$.
Also,~$\omega_i=1$. Suppose, for~$G_{i-1}$,~$\omega_{i-1}$
and~$\omega_{i-1}^v$ are known for all~$v$. Now we will show how~$\omega_i$
and~$\omega_i^v$ can be computed in polynomial-time.

Let~$e_i=(w,w')$. Any new maximum matching resulting from adding~$e_i$ must
contain~$e_i$. Otherwise, all the edges of that matching belong
to~$G_{i-1}$, and therefore, this is a matching in~$G_{i-1}$, a
contradiction. Hence, for vertex~$w$, the number of new matchings it
participates in is exactly equal to the number of new matchings in~$G_i$.
Let~$\alpha_i^v$ denote the number of new maximum matchings that~$v$
participates in. Then, for~$w$,~$p_w(G_i)=\frac{\omega_i^w}{\omega_i}=
\frac{\omega_{i-1}^w+\alpha_i^w}{\omega_{i-1}+\alpha_i^w}$.
Given~$p_w(G_i)$,~$\alpha_i^w$ can be computed using the above expression.
Subsequently,~$\omega_i$ and~$\omega_{i}^w$ can be computed as well. For
any~$v\ne w,w'$,~$p_v(G_i)=\frac{\omega_i^v}{\omega_i}=
\frac{\omega_{i-1}^v+\alpha_i^v}{\omega_i}$. Therefore,~$\alpha_i^v$ and
subsequently~$\omega_i^v$ can be computed using the above expression.

Therefore, the number of maximum matchings in~$G$ can be computed in
polynomial-time.
\QED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi
%the case when the compatibility function is a single disjunction
%nd the class \compatibilityset{} is also a single disjunction.

%After presenting this proof, we will indicate the necessary
%modifications to obtain the result for the case when
%the compatibility function is a single conjunction
%and the class \compatibilityset{} is also a single conjunction.
We study three types of advice frameworks motivated by 
real-world applications. In each case, the compatibility functions
are special cases of monotone-CNF functions. The first
class~$\frameworkor$ corresponds to the framework where~$\kappa_i$ is a
disjunction of variables. In this case,~resource~$y_j$ is compatible
with~$x_i$ if~$y_j$ has at least one attribute value whose corresponding
variable is present in~$\Gamma_i$ (the set of variables used
in $\kappa_i$).
%i.e.,~$\kappa_i(\attvec(y_j))=1$
%iff~$\Gamma_i\cap B_j\ne \varnothing$. 
The second class~$\frameworkand$
corresponds to the framework where~$\kappa_i$ is a conjunction of variable.
A resource~$y_j$ is compatible with~$x_i$ iff~
%$\Gamma_i\subseteq B_j$, or
%in other words, 
the resource has all properties that the agent desires.

The third type of framework is the \emph{conjunction of threshold
functions}. Let $\mathbb{R}$ denote the set of real numbers.
A \textbf{threshold} function 
$g_{\tau} \,:\, \mathbb{R} \rightarrow \{0,1\}$
is characterized by a non-negative threshold value $\tau$; for any
$t \in \mathbb{R}$,
$g_{\tau}(t) = 1$ if $t \geq \tau$ and 0 otherwise.
%for consists of a non-negative real-value
%called threshold. The input to the function is again a non-negative
%real-value. The function returns true iff the input is greater than or
%equal to the threshold. 
In our setting, we assume that the variables of
every attribute have a natural ordering, say~$b_1<b_2<\cdots$. 
For every resource~$y_j$, the attribute function satisfies the following
condition:~$b_k=1$ implies
that~$b_{k-1}=1$, for all $k \geq 2$.
We refer to this attribute function as~$\attvecth$.  For
agent~$x_i$,~$b_k\in \Gamma_i$ implies that~$b_{k-1}\in \Gamma_i$. 
We refer
to this class of functions as~$\compatth$.  
For~$y_j$,
let~$b_{\min}^j=\argmax_{b_k} b_k=1$ and let threshold of~$x_i$
be~$\tau_i=\argmin_{b_k} b_k\in \Gamma_i$. 
It is easy to see that the clause
is true iff~$\tau_i\ge b_{\min}^j$. Finally, we define a monotone cost
function~$\chith(b_k)$ as the cost of changing the threshold to~$b_k$. It has the following property, $\forall b,b'\in \boolattribs$, $b<b'$
implies~$\chith(b)>\chith(b')$. 
The rationale behind this cost function is
that the more one deviates from the threshold, 
the larger is the cost. The
threshold framework comprises of these components and is denoted
by~$\frameworkth(\forbidden,\attvecth,\compatth,\kappa_i,\chith)$.


%% \paragraph{Bithreshold functions~$\compatth$.}
%% This class corresponds to 
%% Another class of compatibility functions that we consider is the
%% conjunction of threshold functions.  While on the outset this setting
%% does not correspond to a Boolean formula in CNF form, there are certain
%% scenarios which can be modeled as threshold functions. This is described
%% below. Suppose for an attribute~$a$ the possible values
%% are~$V_a=\{a(1),a(2),\ldots\}$ such that~$a(1)<a(2)<\cdots$. The attribute
%% set of every resource~$y_i$ satisfies the following property: For
%% every~$k>1$,~$a(k)\in A_i$ implies that~$a(k-1)\in A_i$. For an
%% agent~$x_j$, the set of Boolean variables~$\Gamma_i$ used in it's
%% compatibility function satisfies the following property: For
%% every~$k<|V_a|$, $a(k)\in \Gamma_i$ implies that~$a(k+1)\in \Gamma_i$.
%% Set~$a_{\min}^i=\max a(k)\in A_i$ and the threshold of~$\kappa_j$ is
%% $t(a,j)=\min a(k)\in \Gamma_i$. The clause corresponding to attribute~$a$
%% is true iff~$t(a,j)\ge a_{\min}^i$.

We give an example of the threshold system described above in the
context of the course-classroom example.  Suppose we have only the capacity attribute. We can order the variables in this example as
follows:~$c_{10}<c_{20}<\cdots<c_{50}$. Recall from Example~1 that the capacity of~$y_1$ is~$40$. This means that~$\attvec(y_1)=(1,1,1,1,0)$.
For a course~$x_1$, suppose the minimum capacity requirement is~$30$,
then,~$\kappa_i= {50}(c_{30}\Or c_{40}\Or c_)$.
Clearly,~$x_1$ is compatible with~$y_1$.

%\smallskip

\noindent
\textbf{Estimating number of maximum matchings.}~ Algorithms for finding a
maximum matching and enumerating all maximum matchings in bipartite graphs
form an important component of our advice generation methods. We have two
requirements: the \prin{} needs to (i)~sample uniformly from the space of
maximum matchings of the compatibility graph for assigning resources to
agents, and (ii)~compute the probability that an agent will be matched in
such a maximum matching.
%Both problems are known
%to be hard~\cite{}. 
%\textcolor{red}{(We need to think about the next sentence
%that informally talks about the hardness of (i) and (ii) above. I thought %that (i) is not difficult.)}
These problems are closely related to the computationally difficult problem
of counting the number of maximum matchings in bipartite graphs
\cite{Jerrum-1987,miklos2020counting}.  Therefore, we use use the following
heuristic methods in our experiments.  For~(i), we use the following method
based on the matching algorithm by Hopcroft and
Karp~(\citeyear{Hopcroft-Karp-1973}). We randomly permute the node labels
of~$V_{\sagset}$, apply this algorithm to find a maximum matching, and
apply the inverse of the permutation to obtain the original labels. We
refer to this as the \emph{random HK-algorithm} (\rhk{} algorithm).
For~(ii) we use a combination of \rhk{} algorithm and the iterative
algorithm developed by Uno~(\citeyear{uno1997algorithms})
to enumerate all maximum matchings in a bipartite graph, which we refer to
as the \hkuno{} algorithm.  Let~$\trueprob$ be the probability that~$x_i$
is matched. The notation \hkuno{}$(\nhk,\nuno)$ corresponds to~$\nhk$
iterations of first running~\rhk{} algorithm followed by running the Uno
algorithm for ~$\nuno$ steps. This which will provide~$\nhk(\nuno+1)$
matchings, and we keep track of how many of these matchings contain $x_i$.
From these values, we can compute an empirical estimate $\empprob$
of~$\trueprob$.  Using appropriate values of $\nhk$ and $\nuno$, we will
refer to \hkuno{}$(\nhk,\nuno)$ as the ``matching oracle".

Here, we have two attributes ($\alpha=2$).  
We will encode the attribute
values as Boolean
variables:~$\boolattribs=\{c_{10},c_{20},\ldots,c_{50},r_1,r_2,r_3,r_4\}$,
where the '$c$' corresponds to capacity and '$r$' to region. 
Let~$y_1$ be a
classroom in region~1 with maximum capacity~$40$ and~$y_2$ be a classroom
in region~4 that can accommodate courses of size between~$40$ and~$50$.
Then, for the 
ordering~$\langle c_{10},c_{20},\ldots,c_{50},r_1,r_2,r_3,r_4 \rangle$, the attribute vectors of $y_1$ and $y_2$ are $\attvec(y_1)=(1,1,1,1,0,1,0,0,0)$
and~$\attvec(y_2)=(0,0,0,1,1,0,0,0,1)$, respectively.  
Suppose the instructor
for the course~$x_1$ would like to have a classroom in region~$1$ or~$3$
and with capacity in the range~$20$ and~$30$. The corresponding
compatibility function is 
$\kappa_1=(c_{20}\Or c_{30})\And (r_1 \Or r_3)$. 
%where~$\And$ and $\Or$ are the logical AND and OR operators
%respectively.  
Note that~$x_1$ is compatible with $y_1$; 
in fact, $x_1$'s preferences satisfy both the capacity and region
constraints of $y_1$.
However, $x_1$ is not compatible with ~$y_2$.
Here, the function $\kappa_1$ is from the class ~$\compatibilityset$ corresponding to monotone-CNF functions
with one clause per attribute.
%%
%% \begin{observation}\label{obs:compatibility_equivalence}
%% For an agent~$x$, consider the set of distinct compatibility 
%% functions~$\kappa_i=\{f(\cdot)\mid \exists y \in Y\ s.t.\ f=\kappa_{x,y}\}$.
%% Clearly, there exist at most~$n_y$ different~$\kappa_{x,y}$ functions.
%% The compatibility function partitions resources in~$Y$ into equivalence
%% classes. If~$y$ and~$y'$ have the same compatibility function, then, for
%% removal of certain restrictions,~$y$ becomes compatible with~$x$ iff~$y'$
%% becomes compatible with~$x$.
%% \end{observation}

\paragraph{Forbidden resources for an agent.} In many scenarios, it is
natural that even compatible resources for an agent might be off limits
(e.g., a classroom in one department may not be assigned to a course
offered by a different department). One
can represent such situations by carefully encoding the
agent's compatibility function or changing the attribute sets of such
resources. Here, we find it more convenient to introduce the concept of
a \textbf{forbidden set} of resources~$\forbidden$ 
for each agent~$x_i$. 
For any~$y_j\in\forbidden$, 
the edge~$\{x_i,y_j\}$ will never be added to the
compatibility graph.


%%
\paragraph{Suggesting changes to~$\kappa_i$ through extensions.} The
objective is to suggest modifications to the compatibility function in such
a way that any resource that is already compatible (but unmatched)
continues to be compatible with the agent, and additional resources become
compatible as a result of the modifications.
Such modifications increase the chances
of the agent being matched. Therefore, we will consider only modifications that
satisfy the following property: $\kappa'_i$ is an \textbf{extension}
of~$\kappa_i$; i.e., for any input~$\attvec$,~$\kappa_i(\attvec)=1$ implies that~$\kappa'_i(\attvec)=1$. 
Since we want such extensions to be meaningful under the
advice framework, 
in this paper we restrict our study to
extensions that belong to the same class as~$\kappa_i$;
i.e.,~$\kappa_i,\kappa'_i\in\compatibilityset$, for some
class~$\compatibilityset$.

Continuing with our course-classroom example, there are two ways to obtain
an extension of~$\kappa_1$: we can either add more variables to a clause or remove a clause. For instance, 
$\kappa'_1= (c_{20}\Or c_{30}\Or c_{40})$ 
is an extension of~$\kappa_1$ considered in Example~1.
It was obtained by adding the 
variable~$c_{40}$ to the first clause (that specifies
preferences for set capacities for the course)
and removing the region preferences. 
Now,~$x_1$ is compatible with~$y_2$ also.

\paragraph{Cost and benefit of extending~$\kappa_i$.} For each variable~$b\in
\boolattribs$, we will assign a cost~$\chi(b)$ for either adding it to or
removing it from~$\kappa_i$ depending on the context. If~$b$ is untouched, then, no cost is incurred. 
If $\Gamma_i$ and $\Gamma'_i$ denote the set of variables that
are in $\kappa_i$ and $\kappa'_i$ respectively,
The total cost incurred by the extension $\cost(\kappa'_i)$ is 
given by $\sum_{b \in (\Gamma'_i \,\Delta\, \Gamma_i)} \chi(b)$,
where `$\Delta$' represents the symmetric difference operator.
%the sum of the costs incurred for each~$b\in
%\boolattribs$:~$\cost(\kappa'_i)=
%\sum_{b\in\Gamma'\setminus\Gamma}\chi(b)$.
The benefit of extending~$\kappa_i$ to~$\kappa'_i$ is equal to the number of new maximum matchings in which~$x_i$ is matched.
Let~$\benefit(\kappa_i)$ denote this value.

We are now ready to define formally the advice framework. Given a set of
agents~$\agset$, resources~$\rset$, attribute value set~$\boolattribs$ and
the compatibility graph~$G(V_\agset,V_\rset,E)$, the advice framework
for agent~$x_i$ is denoted
by~$\framework(\forbidden,\attvec,\compatibilityset,\kappa_i,\chi)$,
where~$\forbidden$ is the set of forbidden resources,~$\attvec(\cdot)$ is
the attribute function,~$\compatibilityset$
is the function class of allowed compatibility functions,~$\kappa_i$ is the
current compatibility function of~$x_i$ and~$\chi(\cdot)$ is the cost
function. Now we define the \problem{} problem.

\begin{definition}[Problem {\normalfont \problem}]
For a customer~$x_i\in X$ with advice
framework~$\framework(\forbidden,\attvec,
\compatibilityset,\kappa_i,\chi)$ and
budget~$\beta$, find~$\kappa^*_i\in \compatibilityset$ that maximizes benefit with cost $\leq$ $\beta$; i.e.,~$\kappa^*_i=\argmax_{\kappa'_i\in
\compatibilityset}\benefit(\kappa'_i)$ and~$\cost(\kappa^*_i)\le\beta$.
\end{definition}

Each agent~$x_i$ expresses its preferences as a Boolean formula $\kappa_i$
that uses a subset~$\Gamma_i$ of~$\boolattribs$.  We refer to $\kappa_i$ as
the \textbf{compatibility function} of agent $x_i$.  Formally,
~$\kappa_i:\{0,1\}^{|\boolattribs|}\rightarrow\{0,1\}$, is a function which
takes a binary vector of length~$|\boolattribs|$ as input; it assigns to
each variable in~$\Gamma_i$ the value in the input vector that corresponds
to this variable and produces a Boolean value as output.  Using this
notation, we say that a resource $y_j$ with attribute vector~$\attvec(y_j)$
is \textbf{compatible} with~$x_i$ iff~$\kappa_i(\attvec(y_j))=1$. We will
assume that~$\kappa_i$ belongs to a class of Boolean functions,
say~$\compatibilityset$.

Formally, let~$\agset =\{x_1,x_2,\ldots, x_n\}$ be a set of~$n$ agents
and~$\rset =\{y_1,y_2,\ldots, y_m\}$ be a set of~$m$ resources. Each
resource is characterized by a finite set of~$\alpha$ attributes. It is
assumed that each attribute can take on a finite set of discrete values; by
suitable encoding, one can ensure that the sets of values for any pair of
attributes are disjoint.  (We will present an example of such an encoding
below.) Each attribute value is associated with a Boolean variable, which
is set to~$1$ for a resource only if the resource has that attribute value.
Let~$\boolattribs$ be the collection of all such Boolean variables.
Let~$\attvec:\rset\rightarrow \{0,1\}^{|\boolattribs|}$ be the
representation of the attribute values of a resource in a binary vector form for
some standard ordering of the variables in~$\boolattribs$.
The position corresponding to~$b\in\boolattribs$ in~$\attvec(y_j)$ is set to 1 if $y_j$ has the value corresponding to~$b$; it is
set to 0 otherwise.
Suppose~$x\in\agset$ and $y\in\rset$ are currently
incompatible due to a minimal set of
restrictions~$C=\{c_1,c_2,\ldots,c_\ell\}$. We draw an edge in~$H$
between~$x$ and~$y$ with edge labels in this set. It is possible that there
exists another minimal set of restrictions~$C'$, which when relaxed,~$x$
and~$y$ become compatible. In such cases, we will have multi-edges
between~$x$ and~$y$, one for each set of restrictions. If~$x$ and~$y$ are
compatible, there is a single edge between them without any labels.
The subgraph of unlabeled edges of the restrictions graph is called the
\emph{compatibility} graph denoted by~$G(\agset,\rset,E)$; it is the
bipartite graph i.e., . A \emph{bipartite graph} $G(\agset,
\rset, E)$, where the node sets \agvset{} and \rvset{} correspond to
agents and resources respectively and each edge $\{u,v\} \in E$, with $u
\in \agvset$ and $v \in \rvset$, indicates that the agent represented by
$u$ is compatible with the resource represented by $v$.  We refer to $G$ as
the \textbf{compatibility graph}.

Numbers:
AND: Average(maximum(0,Exhaustive probability - Greedy))=0.016, stdev= 0.06837. min(pi +)  for the greedy and exhaustive algorithm were 0, 0  and max values were 1 and 1.
OR: Average(maximum(0, Exhaustive probability - Greedy))=0.0085, stdev= 0.01256. min(pi +) for the greedy and exhustive algorithm were 0.502 and 0.485 and max values were 1 and 1.
The parameters with greatest covariance were B (0.02 in AND and 0.0007 in OR) and resources_amount( -0.03 and 0.0036) .
For the AND case I run ~300 experiments when setting the other parameters to some constant value. I found that when the world (B) is greater, the error is also greater. I couldn't have the same findings on the OR case since the greedy and the exhaustive gave very similar probabilities.
A graph for the AND case with |B| as the X axis, is available on the sup_figures folder(with some more heatmaps and the graph with the distinct number of resources per 100 when having different amounts of attributes and values).

Parameters that were used for the AND case for verifying the effect of B were:  R=1, Gamma=3, #of resources=40.
and (ii)~evaluation of the algorithms developed for the \problem{} under
different explanation frameworks.

\begin{figure}[t]
\centering
\begin{tabular}{cc}  
\includegraphics[height=2.5cm,width=0.5\linewidth]{figures/theta1_change_2.png}&
\includegraphics[height=2.5cm,width=0.5\linewidth]{figures/theta2_change_2.png}\\
\multicolumn{2}{c}{\includegraphics[height=2.5cm,width=0.5\linewidth]{figures/p_change_2.png}}
\end{tabular}
\caption{Uno vs Hopcroft} 
\label{fig:exp_utility_cmp}
\end{figure}

\begin{itemize}
\item We run each experiment 1000 times
\item Results for 10*10 random graphs were considered. We tried also {5-15}*10 graphs with no important conclusions.
\item For each graph class the parameters for $\theta_hk$ were different.
\item For measuring our results on larger graphs we run the hk-uno algorithm with different parameters on the real dataset and on larger random graphs(e.g., $40*40$ and $80*40$. Here we couldn't calculate the true probabilities because it can take forever. We therefore assumed that lower variance may predict on better parameter set. We found that increasing the number of uno iterations is not improving the variance while the number of hk improves it linearly. That was the reason for using only Hopkroft iterations in the relaxation problem.
\item Runtime of Hopkroft was significantly longer than of a single Uno iteration. HK as a preference because it can run in parallel.
\end{itemize}


\paragraph{Datasets.}
\subsubsection{Children School Vacation.}
A real dataset ~\cite{varone2019dataset}, based on online registration during the summer of 2017 for assigning holiday activities to children.
Each activity has a relevant age range. In addition, dataset contains some children preferences. Some of the activities were very expensive and therefore a child was permitted to participate in them only once in her life. There were three holiday periods in the dataset. Authors suggested a linear program for solving the relevant optimization problem in the case when assigning at most one activity per child is permitted.
\begin{itemize}
\item 634 children participated.
\item there were three vacation period. I picked the one that started at 09/10/2017 0:00 and ended at 15/10/2017 0:00.
\item there were 249 relevant activities in the relevant period (out of 496 in total).
\item Attribute Preferences has the values: 1,2,3,4,5. 1-4 are explicit ratings that provide partial order.
and 5 is when there is no such rating. I assumed that 5 is worse than the other 4 for having a complete order.
\item Attribute min age with values 6-15
\item Attribute max age with values 7-16
\item I did not use the lifetime attribute in the school children case because it was very rare and with no important meaning.
\item There were 3 distinct vacation periods in the graph, I picked one of them.
\item I added all children to the matching.
\item The most relaxed parameter was the preference. In many cases it was relaxed to 5. It means that they need to find a way to increase number of ratings for having better idea about the preferred activities. 
\end{itemize}
\subsubsection{Courses and classrooms graphs}
Although the problem of assigning classrooms to courses is quite common ( e.g., ~\cite{phillips2015integer} ) we couldn't find a dataset that is good for our needs. We collected a new classroom assignment dataset from
a university on 2018-2019 \footnote{Additional information about
the data set will be provided in the final version of the paper}. For each of the 144 classrooms, a region in the university and total student capacity is given. In addition, each classroom has details about its available disability accessories. For many of the courses there were specific region preferences. Since we couldn't find real details about people with disability, we generated the relevant data randomly, giving a course 10 percents for needing one of the accessories and 1 percent for needing both.

\begin{itemize}
\item We have the Capacity attribute with values from 16 to 270
\item there are also the region attributes with values {1100,900,200,400,500,300,100,1000 }
\item As discussed, their order was determined randomly.
 
\the hearing and accessible attributes were generated randomly as before.

\item 144 rooms
\item I picked all courses that used at least part of the window of Tuesday, 14:00 pm- 16:00 pm.
\item I filtered out randomly about 40 percents of the rooms for having lower matching probabilities.
\item The administrator said that they have to keep 20 percents of the rooms empty for some events.
\item The initial number of courses in the time-range is 154.

\end{itemize}

\subsection{Evaluating \hkuno{} algorithm.}

The main objective was to assess the quality of the algorithm.
For the \rhk{} algorithm, we used the implementation of the python NetworkX package~(\citeyear{SciPyProceedings_11}). For the Uno~(\citeyear{uno1997algorithms}) iterations, we used a github implementation. \footnote{https://github.com/Xunius/bipartite\textunderscore matching} as a basis. For making the implementation simple we did not implement the suggested speed up improvements.
For measuring the quality of the \rhk{} algorithm and determining its parameters we generated a large set of random graphs. Graphs differ in their $P$ values, which is the probability of an edge to exist. They also differ in the number of the nodes in each of their parts. For each graph and for each of its nodes, the ~$\empprob$ was calculated by using \rhk{} with different parameters. The results were averaged over multiple nodes and multiple graphs and compared to the ~$\trueprob$ by using the Uno~(\citeyear{uno1997algorithms}) algorithm. 
\begin{figure}
\includegraphics[height=6cm,width=9cm]{figures/0.35_10_10_1000.png}
\caption{An example heatmap that shows the Average MSE in a set of $1000$ random graphs with $P=0.35$, $n=10$ and $m=10$. The y axis represents $\nhk$ and the x axis represents $\nuno$. The brighter squares indicate greater mistakes. }
\end{figure}

\subsection{Performance of the algorithms for calculating ~$\frameworkand$\label{alg:and_greedy} and ~$\frameworkand$\label{alg:or_greedy} on synthetic graphs.}
\begin{itemize}
\item For both the AND and OR cases, I used the parameters: R= values per Attribute,{1..5}
                       B= world size, {2,4,6,8,10,12}
                       Gamma= preferences size, { 1..5 }
                       Resources amount, {20,40}
                       Budget { 1...5 }
                       
\item for the AND case, the average difference between the greedy heuristic and the exhustive search was 0.02 for all 6921 experiments. 
\item In my implementation, I called the oracle for each set of relaxed resources (1 or more) without checking if it increased the matching size.
\item In the OR case there was no significant difference. Actually the greedy was better in 0.001 percents (negligible because of the error).
\Item I found that as the world (B) is greater, the error is also greater.

\end{itemize}                       

\subsection{Performance of the algorithm for calculating ~$\frameworkth$\label{alg:thresh} on the real datasets.}
>>>>>>> 9b9805c8d9813b8318c8eabf60ef4957b5e7121e

\begin{itemize}
\item I picked all courses that used at least part of the window of Tuesday, 14:00 pm- 16:00 pm.
\item I filtered out randomly about 40 percents of the rooms for having lower matching probabilities.
\item The administrator said that they have to keep 20percents of the rooms empty for some events.
\item The initial number of courses in the time-range is 154.

\end{itemize}
%% Some of the activities were very expensive and therefore a
%% child was permitted to participate in them only once in her life. There
%% were three holiday periods in the dataset. Authors suggested a linear
%% program for solving the relevant optimization problem in the case when
%% assigning at most one activity per child is permitted.
%% \begin{itemize}
%% \item Attribute Preferences has the values: 1,2,3,4,5. 1-4 are explicit ratings that provide partial order.
%% and 5 is when there is no such rating. I assumed that 5 is worse than the other 4 for having a complete order.
%% \item Attribute min{\_}age with values 6-15
%% \item Attribute max{\_}age with values 7-16
%% \item I did not use the lifetime attribute in the school children case because it was very rare and with no important meaning.
%% \item There were 3 distict vacation periods in the graph, I picked one of them.
%% \item I added all children to the matching.
%% \end{itemize}

\begin{itemize}
\item We run each experiment 1000 times
\item Results for 10*10 random graphs were considered. We tried also {5-15}*10 graphs with no important conclusions.
\item For each graph class the parameters for $\theta_hk$ were different.
\item For measuring our results on larger graphs we run the hk-uno algorithm with different parameters on the real dataset and on larger random graphs(e.g., $40*40$ and $80*40$. Here we couldn't calculate the true probabilities because it can take forever. We therefore assumed that lower variance may predict on better parameter set. We found that increasing the number of uno iterations is not improving the variance while the number of hk improves it linearly. That was the reason for using only Hopkroft iterations in the relaxation problem.
\item Runtime of Hopkroft was significantly longer than of a single Uno iteration. HK as a preference because it can run in parallel.
\end{itemize}


The main objective was to assess the quality of the algorithm.  For the
\rhk{} algorithm, we used the implementation of the python NetworkX
package~(\citeyear{SciPyProceedings_11}) and for the ``Uno'' component of
the algorithm we used a github
implementation\footnote{https://github.com/Xunius/bipartite\textunderscore
matching} as a basis. For making the implementation simple we did not
implement the suggested speed up improvements.  For measuring the quality
of the \rhk{} algorithm and determining its parameters we generated a large
set of random
graphs. Graphs differ in their $P$ values, which is the probability of an
edge to exist. They also differ in the number of the nodes in each of their
parts. For each graph and for each of its nodes, the ~$\empprob$ was
calculated by using \rhk{} with different parameters. The results were
averaged over multiple nodes and multiple graphs and compared to the
~$\trueprob$ by using the Uno~(\citeyear{uno1997algorithms}) algorithm.

Parameter sets for both AND and OR cases:
R= values per Attribute,{1..5}
B= world size, {2,4,6,8,10,12}
Gamma= preferences size, { 1..5 }
Resources amount, {20,40}
Agents amount, {40 for 20 resources and 80 for 40 resources}
Budget { 1...5 }

